Self-consistent electron lifetimes for electron-phonon scattering

Acoustic phonons in piezoelectric materials strongly couple to electrons through a macroscopic electric field. We show that this coupling leads to a momentum-dependent divergence of the Fan-Migdal electron linewidth. We then develop a self-consistent theory for calculating electron linewidths, which not only removes this piezoelectric divergence but also considerably modifies the linewidth in nonpiezoelectric, polar materials. Our predictions await immediate experimental confirmation, and this self-consistent method should be broadly used in interpreting various experiments on the electronic properties of real materials.

==> xx.tex <==



==> xy.tex <==


